Self-Supervised Unseen Object Instance Segmentation via Long-Term Robot Interaction

We introduce a novel robotic system for improving unseen object instance segmentation in the real world by leveraging long-term robot interaction with objects. Previous approaches either grasp or push an object and then obtain the segmentation mask of the grasped or pushed object after one action. Instead, our system defers the decision on segmenting objects after a sequence of robot pushing actions. By applying multi-object tracking and video object segmentation on the images collected via robot pushing, our system can generate segmentation masks of all the objects in these images in a self-supervised way. These include images where objects are very close to each other, and segmentation errors usually occur on these images for existing object segmentation networks. We demonstrate the usefulness of our system by fine-tuning segmentation networks trained on synthetic data with real-world data collected by our system. We show that, after fine-tuning, the segmentation accuracy of the networks is significantly improved both in the same domain and across different domains. In addition, we verify that the fine-tuned networks improve top-down robotic grasping of unseen objects in the real world.

==> experiments_across.tex <==

\begin{table*}[!ht]
\caption{UOIS results on the OCID and OSD datasets. * indicates a model after fine-tuning. \yu{add citation}}\label{all_results}
\centering
\scalebox{1.0}{
\begin{tabular}{|l|l|lllllll|lllllll|}
\hline
\multirow{3}{*}{Method}    & \multirow{3}{*}{Input} & \multicolumn{7}{c|}{OCID (2390 images)}                                                                                                                                                 & \multicolumn{7}{c|}{OSD (111 images)}                                                                                                                                                   \\ \cline{3-16} 
                           &                        & \multicolumn{3}{c|}{Overlap}                                                       & \multicolumn{3}{c|}{Boundary}                                                      &               & \multicolumn{3}{c|}{Overlap}                                                       & \multicolumn{3}{c|}{Boundary}                                                      &               \\
                           &                        & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F}             & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F}             & \%75          & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F}             & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F}             & \%75          \\ \hline
MRCNN                      & \multirow{10}{*}{RGB}   & 77.6                  & 67.0                  & \multicolumn{1}{l|}{67.2}          & 65.5                  & 53.9                  & \multicolumn{1}{l|}{54.6}          & 55.8          & 64.2                  & 61.3                  & \multicolumn{1}{l|}{62.5}          & 50.2                  & 40.2                  & \multicolumn{1}{l|}{44.0}          & 31.9          \\
UCN                        &                         & 54.8                  & 76.0                  & \multicolumn{1}{l|}{59.4}          & 34.5                  & 45.0                  & \multicolumn{1}{l|}{36.5}          & 48.0          & 57.2                  & \textbf{73.8}         & \multicolumn{1}{l|}{63.3}          & 34.7                  & 50.0                  & \multicolumn{1}{l|}{39.1}          & 52.5          \\
UCN + Zoom-in              &                         & 59.1                  & 74.0                  & \multicolumn{1}{l|}{61.1}          & 40.8                  & 55.0                  & \multicolumn{1}{l|}{43.8}          & 58.2          & 59.1                  & 71.7                  & \multicolumn{1}{l|}{63.8}          & 34.3                  & 53.3                  & \multicolumn{1}{l|}{39.5}          & 52.6          \\
Mask2Former\_R50           &                         & 67.2                  & 73.1                  & \multicolumn{1}{l|}{67.1}          & 55.9                  & 58.1                  & \multicolumn{1}{l|}{54.5}          & 54.3          & 60.6                  & 60.2                  & \multicolumn{1}{l|}{59.5}          & 48.2                  & 41.7                  & \multicolumn{1}{l|}{43.3}          & 32.4          \\
MSMFormer\_R50             &                         & 72.9                  & 68.3                  & \multicolumn{1}{l|}{67.7}          & 60.5                  & 56.3                  & \multicolumn{1}{l|}{55.8}          & 52.9          & 63.4                  & 64.7                  & \multicolumn{1}{l|}{63.6}          & 48.6                  & 47.4                  & \multicolumn{1}{l|}{47.0}          & 40.2          \\
MSMFormer\_R50 * (Ours)    &                         & 80.3                  & 81.0                  & \multicolumn{1}{l|}{78.5}          & 67.9                  & 70.8                  & \multicolumn{1}{l|}{67.4}          & 73.1          & 63.5                  & 71.7                  & \multicolumn{1}{l|}{66.8}          & 44.8                  & 56.2                  & \multicolumn{1}{l|}{48.7}          & 49.8          \\
MSMFormer\_R50 +Zoom-in    &                         & 73.9                  & 67.1                  & \multicolumn{1}{l|}{66.3}          & 64.6                  & 52.9                  & \multicolumn{1}{l|}{54.8}          & 52.8          & 63.9                  & 63.7                  & \multicolumn{1}{l|}{62.7}          & 51.6                  & 45.3                  & \multicolumn{1}{l|}{47.0}          & 41.1          \\
MSMFormer\_R50 + Zoom-in*  &                         & 76.6                  & 71.1                  & \multicolumn{1}{l|}{70.4}          & 68.1                  & 57.8                  & \multicolumn{1}{l|}{59.8}          & 58.7          & \textbf{69.8}         & 69.1                  & \multicolumn{1}{l|}{\textbf{69.0}} & \textbf{54.8}         & 52.2                  & \multicolumn{1}{l|}{\textbf{52.5}} & 50.7          \\
MSMFormer\_R50* + Zoom-in  &                         & 79.5                  & 77.1                  & \multicolumn{1}{l|}{75.5}          & 68.9                  & 64.8                  & \multicolumn{1}{l|}{64.6}          & 68.3          & 63.4                  & 71.5                  & \multicolumn{1}{l|}{66.6}          & 47.0                  & 55.0                  & \multicolumn{1}{l|}{49.4}          & 52.0          \\
MSMFormer\_R50* + Zoom-in* &                         & \textbf{83.5}         & \textbf{82.1}         & \multicolumn{1}{l|}{\textbf{80.6}} & \textbf{74.1}         & \textbf{72.5}         & \multicolumn{1}{l|}{\textbf{71.7}} & \textbf{77.9} & 66.2                  & 72.3                  & \multicolumn{1}{l|}{68.4}          & 50.3                  & \textbf{56.8}         & \multicolumn{1}{l|}{52.0}          & \textbf{56.0} \\ \hline
MRCNN                      & \multirow{3}{*}{Depth}  & 85.3                  & 85.6                  & \multicolumn{1}{l|}{84.7}          & 83.2                  & 76.6                  & \multicolumn{1}{l|}{78.8}          & 72.7          & 77.8                  & 85.1                  & \multicolumn{1}{l|}{80.6}          & 52.5                  & 57.9                  & 54.6                               & 77.6          \\
UOIS-Net-2D {[}33{]}       &                         & 88.3                  & 78.9                  & \multicolumn{1}{l|}{81.7}          & 82.0                  & 65.9                  & \multicolumn{1}{l|}{71.4}          & 69.1          & 80.7                  & 80.5                  & \multicolumn{1}{l|}{79.9}          & 66.0                  & 67.1                  & 65.6                               & 71.9          \\
UOIS-Net-3D {[}34{]}       &                         & 86.5                  & 86.6                  & \multicolumn{1}{l|}{86.4}          & 80.0                  & 73.4                  & \multicolumn{1}{l|}{76.2}          & 77.2          & 85.7                  & 82.5                  & \multicolumn{1}{l|}{83.3}          & 75.7                  & 68.9                  & 71.2                               & 73.8          \\ \cline{2-2}
MRCNN                      & \multirow{11}{*}{RGB-D} & 79.6                  & 76.7                  & \multicolumn{1}{l|}{76.6}          & 68.7                  & 63.7                  & \multicolumn{1}{l|}{64.3}          & 62.9          & 66.4                  & 64.8                  & \multicolumn{1}{l|}{65.5}          & 53.7                  & 43.8                  & 47.5                               & 37.1          \\
UCN                        &                         & 86.0                  & \textbf{92.3}         & \multicolumn{1}{l|}{88.5}          & 80.4                  & 78.3                  & \multicolumn{1}{l|}{78.8}          & 82.2          & 84.3                  & \textbf{88.3}         & \multicolumn{1}{l|}{86.2}          & 67.5                  & 67.5                  & 67.1                               & 79.3          \\
UCN + Zoom-in              &                         & 91.6                  & 92.5                  & \multicolumn{1}{l|}{91.6}          & 86.5                  & \textbf{87.1}         & \multicolumn{1}{l|}{86.1}          & \textbf{89.3} & 87.4                  & 87.4                  & \multicolumn{1}{l|}{\textbf{87.4}} & 69.1                  & 70.8                  & 69.4                               & 83.2          \\
UOAIS-Net                  &                         & 70.7                  & 86.7                  & \multicolumn{1}{l|}{71.9}          & 68.2                  & 78.5                  & \multicolumn{1}{l|}{68.8}          & 78.7          & 85.3                  & 85.4                  & \multicolumn{1}{l|}{85.2}          & \textbf{72.7}         & \textbf{74.3}         & \textbf{73.1}                      & 79.1          \\
Mask2Former                &                         & 78.6                  & 82.8                  & \multicolumn{1}{l|}{79.5}          & 69.3                  & 76.2                  & \multicolumn{1}{l|}{71.1}          & 69.3          & 75.6                  & 79.2                  & \multicolumn{1}{l|}{77.3}          & 54.1                  & 64.0                  & 58.0                               & 65.2          \\
MSMFormer                  &                         & 88.4                  & 90.2                  & \multicolumn{1}{l|}{88.5}          & 84.7                  & 83.1                  & \multicolumn{1}{l|}{83.0}          & 80.3          & 79.5                  & 86.4                  & \multicolumn{1}{l|}{82.8}          & 53.5                  & 71.0                  & 60.6                               & 79.4          \\
MSMFormer * (Ours)         &                         & 91.2                  & 90.1                  & \multicolumn{1}{l|}{90.1}          & 87.2                  & 85.5                  & \multicolumn{1}{l|}{85.7}          & 83.9          & 85.1                  & 84.4                  & \multicolumn{1}{l|}{84.6}          & 67.8                  & 71.4                  & 69.0                               & 76.2          \\
MSMFormer + Zoom-in        &                         & 92.5                  & 91.0                  & \multicolumn{1}{l|}{91.5}          & 89.4                  & 85.9                  & \multicolumn{1}{l|}{87.3}          & 86.0          & 87.1                  & 86.1                  & \multicolumn{1}{l|}{86.4}          & 69.0                  & 68.6                  & 68.4                               & \textbf{80.4} \\
MSMFormer + Zoom-in*       &                         & 91.3                  & 91.3                  & \multicolumn{1}{l|}{91.0}          & 87.7                  & 84.4                  & \multicolumn{1}{l|}{85.6}          & 86.2          & 86.6                  & 82.9                  & \multicolumn{1}{l|}{84.4}          & 68.9                  & 69.6                  & 68.6                               & 76.3          \\
MSMFormer* + Zoom-in       &                         & \textbf{92.7}         & 91.6                  & \multicolumn{1}{l|}{\textbf{91.9}} & \textbf{89.9}         & 86.5                  & \multicolumn{1}{l|}{\textbf{87.8}} & 87.1          & 85.5                  & 84.6                  & \multicolumn{1}{l|}{84.8}          & 68.3                  & 65.9                  & 66.7                               & 75.5          \\
MSMFormer* + Zoom-in*      &                         & 91.5                  & 91.8                  & \multicolumn{1}{l|}{91.3}          & 88.2                  & 84.8                  & \multicolumn{1}{l|}{86.1}          & 87.1          & \textbf{87.6}         & 82.6                  & \multicolumn{1}{l|}{84.4}          & 70.8                  & 68.5                  & 68.9                               & 75.8          \\ \hline
\end{tabular}
}
\end{table*}







\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/diff5.png}
\caption{The effect of fine-tuning. \lu{will modify}}
\label{fig:diff}
\end{center}
\end{figure*}

==> experiments_same.tex <==


\begin{table*}[!ht]
\caption{Unseen Object Instance Segmentation results on a same domain dataset. *: the model after Fine-Tuning.}\label{same_domain_Results}
\centering
\scalebox{1.0}{
\begin{tabular}{|l|l|lllllll|}
\hline
\multirow{3}{*}{Method}       & \multirow{3}{*}{Input} & \multicolumn{7}{c|}{Same Domain Dataset (107 images)}                                                                                                                                                 \\ \cline{3-9} 
                              &                        & \multicolumn{3}{c|}{Overlap}                                                       & \multicolumn{3}{c|}{Boundary}                                                      &               \\
                              &                        & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F}             & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F}             & \%75          \\ \hline
MSMFormer\_R50             & \multirow{6}{*}{RGB}       & 81.7                  & 81.7                  & \multicolumn{1}{l|}{81.6}          & 75.7                  & 73.1                  & \multicolumn{1}{l|}{73.7}          & 66.2          \\
MSMFormer\_R50 * (Ours)    &                            & \textbf{90.6}         & \textbf{92.7}         & \multicolumn{1}{l|}{\textbf{91.6}} & \textbf{87.3}         & \textbf{88.6}         & \multicolumn{1}{l|}{\textbf{87.6}} & \textbf{90.7} \\ \cline{1-1} \cline{3-9} 
MSMFormer\_R50 + Zoom-in   &                            & 75.9                  & 81.0                  & \multicolumn{1}{l|}{78.1}          & 68.0                  & 63.7                  & \multicolumn{1}{l|}{65.1}          & 61.6          \\
MSMFormer\_R50 + Zoom-in*  &                            & 90.1                  & 89.6                  & \multicolumn{1}{l|}{89.7}          & 88.0                  & 84.4                  & \multicolumn{1}{l|}{85.5}          & 83.5          \\
MSMFormer\_R50* + Zoom-in  &                            & 83.2                  & 90.9                  & \multicolumn{1}{l|}{86.7}          & 74.4                  & 78.2                  & \multicolumn{1}{l|}{75.8}          & 85.5          \\
MSMFormer\_R50* + Zoom-in* &                            & \textbf{91.0}         & \textbf{93.3}         & \multicolumn{1}{l|}{\textbf{92.1}} & \textbf{89.7}         & \textbf{89.6}         & \multicolumn{1}{l|}{\textbf{89.3}} & \textbf{92.2} \\ \hline
MSMFormer\_R34             & \multirow{6}{*}{RGB-D Add} & 85.8                  & 88.9                  & \multicolumn{1}{l|}{87.2}          & 81.7                  & 78.7                  & \multicolumn{1}{l|}{79.9}          & 75.1          \\
MSMFormer\_R34* (Ours)     &                            & \textbf{90.9}         & \textbf{91.9}         & \multicolumn{1}{l|}{\textbf{91.3}} & \textbf{86.5}         & \textbf{85.9}         & \multicolumn{1}{l|}{\textbf{85.9}} & \textbf{84.8} \\ \cline{1-1} \cline{3-9} 
MSMFormer\_R34 + Zoom-in   &                            & 88.9                  & 89.8                  & \multicolumn{1}{l|}{89.3}          & 86.6                  & 84.4                  & \multicolumn{1}{l|}{85.3}          & 80.7          \\
MSMFormer\_R34 + Zoom-in*  &                            & 90.7                  & 90.2                  & \multicolumn{1}{l|}{90.4}          & 86.0                  & 85.9                  & \multicolumn{1}{l|}{85.6}          & 84.3          \\
MSMFormer\_R34* + Zoom-in  &                            & 91.0                  & \textbf{91.9}         & \multicolumn{1}{l|}{91.3}          & \textbf{89.6}         & 87.2                  & \multicolumn{1}{l|}{88.2}          & 87.0          \\
MSMFormer\_R34* + Zoom-in* &                            & \textbf{92.5}         & \textbf{91.9}         & \multicolumn{1}{l|}{\textbf{92.1}} & 89.3                  & \textbf{87.8}         & \multicolumn{1}{l|}{\textbf{88.3}} & \textbf{88.0} \\  \hline
\end{tabular}
}
\end{table*}
